Code Reviews in Open Source Projects : How Do Gender Biases Affect Participation and Outcomes?

Context: Contemporary software development organizations lack diversity and the ratios of women in Free and open-source software (FOSS) communities are even lower than the industry average. Although the results of recent studies hint the existence of biases against women, it is unclear to what extent such biases influence the outcomes of various software development tasks. Aim: We aim to identify whether the outcomes of or participation in code reviews (or pull requests) are influenced by the gender of a developer.. Approach: With this goal, this study includes a total 1010 FOSS projects. We developed six regression models for each of the 14 dataset (i.e., 10 Gerrit based and four Github) to identify if code acceptance, review intervals, and code review participation differ based on the gender and gender neutral profile of a developer. Key findings: Our results find significant gender biases during code acceptance among 13 out of the 14 datasets, with seven seven favoring men and the remaining six favoring women. We also found significant differences between men and women in terms of code review intervals, with women encountering longer delays in three cases and the opposite in seven. Our results indicate reviewer selection as one of the most gender biased aspects among most of the projects, with women having significantly lower code review participation among 11 out of the 14 cases. Since most of the review assignments are based on invitations, this result suggests possible affinity biases among the developers. Conclusion: Though gender bias exists among many projects, direction and amplitude of bias varies based on project size, community and culture. Similar bias mitigation strategies may not work across all communities, as characteristics of biases and their underlying causes differ.

==> Tables/Model_variables.tex <==


\begin{tabular}{|l|l|l|}
\hline
Model                                                                                   & \begin{tabular}[c]{@{}l@{}}Dependent\\ variable\end{tabular}                       & Independent Variables        \\ \hline
\multirow{10}{*}{\begin{tabular}[c]{@{}l@{}}Acceptance\\ model\end{tabular}}            & \multirow{10}{*}{\begin{tabular}[c]{@{}l@{}}Acceptance\\ rate\end{tabular}}        & Developers experience        \\ \cline{3-3} 
                                                                                        &                                                                                    & Tenure                       \\ \cline{3-3} 
                                                                                        &                                                                                    & Code churn                   \\ \cline{3-3} 
                                                                                        &                                                                                    & Cyclomatic complexity        \\ \cline{3-3} 
                                                                                        &                                                                                    & Number of patchset           \\ \cline{3-3} 
                                                                                        &                                                                                    & Is the commit fixing any bug \\ \cline{3-3} 
                                                                                        &                                                                                    & Number of directory          \\ \cline{3-3} 
                                                                                        &                                                                                    & Comment volume               \\ \cline{3-3} 
                                                                                        &                                                                                    & Is new file                  \\ \cline{3-3} 
                                                                                        &                                                                                    & Gender                       \\ \hline
\multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}Review \\ interval \\ model\end{tabular}}   & \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}Code\\ review\\ interval\end{tabular}} & Developers' experience       \\ \cline{3-3} 
                                                                                        &                                                                                    & Tenure                       \\ \cline{3-3} 
                                                                                        &                                                                                    & Code churn                   \\ \cline{3-3} 
                                                                                        &                                                                                    & Cyclomatic complexity        \\ \cline{3-3} 
                                                                                        &                                                                                    & Number of patch set          \\ \cline{3-3} 
                                                                                        &                                                                                    & If the commit is bug fixing  \\ \cline{3-3} 
                                                                                        &                                                                                    & If it is a new file          \\ \cline{3-3} 
                                                                                        &                                                                                    & Number of files              \\ \cline{3-3} 
                                                                                        &                                                                                    & Number of directory          \\ \cline{3-3} 
                                                                                        &                                                                                    & Comment volume               \\ \cline{3-3} 
                                                                                        &                                                                                    & Gender                       \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Review\\ participation\\ model\end{tabular}} & \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Number of\\ code review\end{tabular}}   & Number of commits            \\ \cline{3-3} 
                                                                                        &                                                                                    & Tenure                       \\ \cline{3-3} 
                                                                                        &                                                                                    & Number of prior reviews      \\ \cline{3-3} 
                                                                                        &                                                                                    & Network degree               \\ \cline{3-3} 
                                                                                        &                                                                                    & Gender                       \\ \hline
\end{tabular}

